Additive domain decomposition operator splittings -- convergence analyses in a dissipative framework

We analyze temporal approximation schemes based on overlapping domain decompositions. As such schemes enable computations on parallel and distributed hardware, they are commonly used when integrating large-scale parabolic systems. Our analysis is conducted by first casting the domain decomposition procedure into a variational framework based on weighted Sobolev spaces. The time integration of a parabolic system can then be interpreted as an operator splitting scheme applied to an abstract evolution equation governed by a maximal dissipative vector field. By utilizing this abstract setting, we derive an optimal temporal error analysis for the two most common choices of domain decomposition based integrators. Namely, alternating direction implicit schemes and additive splitting schemes of first and second order. For the standard first-order additive splitting scheme we also extend the error analysis to semilinear evolution equations, which may only have mild solutions.

==> erik_header.tex <==
% My standard packages and macros.
% Erik Henningsson, 2015.


%%% PACKAGES %%%

\RequirePackage{fix-cm} % Fixes problems like: LaTeX Font Warning: Font shape `OT1/cmr/m/n' in size <X> not available (Is part of the Springer tempelate.)
\usepackage{amsfonts,amsmath,amssymb}
\usepackage{amsthm}											    																															 % SPRINGER COMES WITH ITS OWN ENVIRONMENTS.
\usepackage{graphicx}
\usepackage[IT]{subfigure}
\usepackage{mathrsfs} % Provides a \math­scr command, rather than overwriting the standard \mathcal command. DOESN'T WORK WITH SPRINGER.
\usepackage[usenames,dvipsnames]{color} 			% Not used with BEAMER since BEAMER automatically loads it.
%\usepackage{fixme} 														% Not used with BEAMER since it doesn't work with BEAMER.
%\fxsetup{theme=color} % See mail from Tony below.
%\fxsetup{inline=true,margin=false,marginclue=true} % Good for two-column-articles with little margin space.
\usepackage[exponent-product=\cdot,per-mode=symbol]{siunitx} % \SI{2.3e4}{\kilogram\metre\per\square\second} = \SI{2.3e4}{kg.m/s^2}
\usepackage{ifdraft}

\usepackage[T1]{fontenc} % Note that without this it is not possible to search for å, ä, ö, é, and so on in the pdf file. Additionally, hyphenation can not be made correctly and in general the space between characters are wrong. THIS SHOULD THEREFORE ALWAYS BE INCLUDED, EVEN WHEN WRITING IN ENGLISH. See http://tex.stackexchange.com/questions/664/why-should-i-use-usepackaget1fontenc
\usepackage[utf8]{inputenc} % It should really be latin1 on Windows computers, this works outside the TeXnicCenter project environment, however within the environment latin1 does not work but the Linux variant utf8 works instead. See http://tex.stackexchange.com/questions/44694/fontenc-vs-inputenc % BUT WITH XeLaTeX IT SHOULD FOR SOME REASION BE latin1?!
%\usepackage[latin1]{inputenc} % For XeLaTeX.
\usepackage[swedish,english]{babel} % See http://tex.stackexchange.com/questions/75006/swedish-characters-but-english-captions


%%% SELDOM USED PACKAGES %%%

%\usepackage[framed,numbered,autolinebreaks,useliterate]{mcode/mcode} % For including Matlab code.
%\usepackage{tikz} % For creating images. One of the most advanced packages for this.
%\usepackage{algpseudocode} % For including algorithms
%\usepackage{algorithm} % For including algorithms
%\usetikzlibrary{datavisualization, intersections} % ??? Copied together with the above.
%\usepackage[multidot]{grffile} % For including files with spaces in their names.


%%%% THEOREM ENVIRONMENTS %%%
%
%\newtheoremstyle{assumption}
  %{\topsep}   % ABOVESPACE
  %{\topsep}   % BELOWSPACE
  %{\itshape}  % BODYFONT
  %{0pt}       % INDENT (empty value is the same as 0pt)
  %{\sc} % HEADFONT
  %{.}         % HEADPUNCT
  %{5pt plus 1pt minus 1pt} % HEADSPACE
  %{}          % CUSTOM-HEAD-SPEC
%
%\newtheorem{thm}{Theorem}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{cor}[thm]{Corollary}
%
%\theoremstyle{definition}
%\newtheorem{defi}{Definition}
%\newtheorem{ex}{Example}
%\newtheorem{que_con}{Research topic}
%
%\theoremstyle{remark}
%\newtheorem{rem}{Remark}
%
%\theoremstyle{assumption}
%\newtheorem{as}{Assumption}
%
%\theoremstyle{definition}


%%% MACROS %%%

% Special font letters for sets etc ...
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\RR}{\mathcal{R}}
%\newcommand{\CC}{\mathscr{C}}   % Needs \usepackage{mathrsfs} (included above) but this package doesn't work with Springer.
\newcommand{\CC}{C}
%\newcommand{\CC}{\mathcal{C}}
\newcommand{\Ordo}{\mathcal{O}}
\newcommand{\e}{\mathrm{e}}

% Operators and differentials
\newcommand{\inv}{^{-1}}
\newcommand{\trans}{^{\mathrm{T}}}
\newcommand{\dx}{\:\mathrm{d}x}
\newcommand{\dy}{\:\mathrm{d}y}
\newcommand{\dt}{\:\mathrm{d}t}
\newcommand{\dtau}{\:\mathrm{d}\tau}
\newcommand{\dO}{\:\mathrm{d}\Omega}
\newcommand{\dd}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\newcommand{\ddt}{\frac{\mathrm{d}}{\mathrm{d}t}}
\newcommand{\dede}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dedex}{\dede{}{x}}
\newcommand{\dedey}{\dede{}{y}}

% Environment abbreviations
\newcommand{\bp}{\begin{pmatrix}}
\newcommand{\ep}{\end{pmatrix}}
\newcommand{\bbm}{\begin{bmatrix}}
\newcommand{\ebm}{\end{bmatrix}}

% Miscellaneous: norm and abbreviations
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\norml}[1]{\norm{#1}_{L^2(\Omega)}}
\newcommand{\fp}[2]{\langle #1, #2 \rangle}
\newcommand{\widebar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\vphi}{\varphi}
\newcommand{\ee}[1]{\cdot 10^{#1}}

% Colors
\definecolor{LUbronze}{RGB}{156,97,20}
\definecolor{LUblue}{RGB}{0,0,128}
\definecolor{LUlightblue}{RGB}{185,211,220}
%\definecolor{LUlightblue50}{RGB}{220,233,238} % Probably not correct.

\newcommand{\lubr}[1]{{\color{LUbronze}#1}}
\newcommand{\lubl}[1]{{\color{LUblue}#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\darkgreen}[1]{{\color{green!40!black}#1}}
\newcommand{\darkred}[1]{{\color{red!60!black}#1}}
\newcommand{\orange}[1]{{\color{orange}#1}}
\newcommand{\burntorange}[1]{{\color{BurntOrange}#1}}
\newcommand{\yellow}[1]{{\color{yellow}#1}}
\newcommand{\teal}[1]{{\color{teal}#1}}
\newcommand{\cyan}[1]{{\color{cyan}#1}}
\newcommand{\olive}[1]{{\color{olive}#1}}
\newcommand{\black}[1]{{\color{black}#1}}
\newcommand{\white}[1]{{\color{white}#1}}

% Comments in text and margin, switch on/off
% Rather use the fixme package, confer section 3.2 -- 3.4 of http://ctan.uib.no/macros/latex/contrib/fixme/fixme.pdf
% also don't forget draft vs. final in documentclass
\ifdraft{
\newcommand{\todo}[1]{\marginpar{#1}}
\newcommand{\comment}[1]{\red{\emph{\{#1\}}}} % Fixme defines comment, so with this can't be used together with fixme.
}{
\newcommand{\todo}[1]{}
\newcommand{\comment}[1]{} % Fixme defines comment, so with this can't be used together with fixme.
}


%%% NOTES ABOUT STYLE AND ELSE %%%

% Tony about confer:

% Confer doesn't mean what I think it means. Don't use it like cf., (should I spell out compare then instead?).


% Stefan about capital letters: 

%Man har stor bokstav på Equation när man listar ekvationer: 
	%"Equations (3)-(6)", 
	%Latex: "Equations~\eqref{eq:c}--\eqref{eq:f}".
%Detsamma gäller Figures, Sections, Theorems, Assumptions osv. Man har dock liten bosktav när man skriver
	%"evolution equation (3)".
%Skillnaden är att vi snarare beskriver ekvationen, det är lite som en kortform av
	%"evolution equation Equation (3)".
%Likadant skriver man
	%"model (3)" och
	%"problem (3)"


% Mail from Tony about fixme:

%Jag kör bara
%
%\usepackage{fixme} % Todo notes
%\fxsetup{theme=color}
%
%i preamble, och sen använder man \fxnote{Din text} där note kan bytas ut mot t.ex. error, fatal eller warning. Jag hade lite problem med att justera stilen, färg och sånt, det stämde inte riktigt med manualen. (Potentiellt har jag en gammal version.) Men ovanstående fungerar bra.
%
%För att få en lista i slutet kör man 
%
%\listoffixmes
